Do causal predictors generalize better to new domains?

We study how well machine learning models trained on causal features generalize across domains. We consider 16 prediction tasks on tabular datasets covering applications in health, employment, education, social benefits, and politics. Each dataset comes with multiple domains, allowing us to test how well a model trained in one domain performs in another. For each prediction task, we select features that have a causal influence on the target of prediction. Our goal is to test the hypothesis that models trained on causal features generalize better across domains. Without exception, we find that predictors using all available features, regardless of causality, have better in-domain and out-of-domain accuracy than predictors using causal features. Moreover, even the absolute drop in accuracy from one domain to the other is no better for causal predictors than for models that use all features. In addition, we show that recent causal machine learning methods for domain generalization do not perform better in our evaluation than standard predictors trained on the set of causal features. Likewise, causal discovery algorithms either fail to run or select causal variables that perform no better than our selection. Extensive robustness checks confirm that our findings are stable under variable misclassification.

==> sections/old_sec_discussion.tex <==
\section{Discussion}
Our findings may not come as a surprise to everyone. Unlike causal machine learning researchers, social scientists generally see no reason to believe in the universality of causal relationships. For example, smaller classroom sizes may cause better teaching outcomes in Tennessee~\citep{mosteller1995tennessee}, but much less so in California~\citep{jepsen2009class}. Such variation is the rule rather than the exception. Indeed, philosopher of science~\citet{cartwright1999dappled,cartwright2007hunting} argued that causal regularities are more narrowly scoped than commonly believed. 

Our study mirrors these robust facts in a machine learning context. We find no evidence that causal predictors have greater external validity than their conventional counterparts. If the goal is to generalize to new domains, our findings suggest practitioners might as well train the best possible model on all available features. Put differently, demonstrating the utility of causal methods requires other benchmark datasets than the ones currently available.

We point to two classification tasks, where recent research suggests that causal prediction methods have utility for better domain generalization~\citep{schulam2017pneumonia,subbaswamy2019healthai}. \cite{cooper1997pneumonia} built a predictor for the probability of death for patients with pneumonia. The goal was to identify patients at low risk that can be treated safely at home for pneumonia.
%\footnote{\cite{cooper1997pneumonia} argue that this is likely to reduce the costs of treating pneumonia, and allows patients with mild cases to be treated at home, where they are typically more comfortable.}
Their dataset contains inpatient information from 78 hospitals in 23~U.S.~States.
% from the 1989 MedisGroups Comparative Hospital Database
~\cite{cooper1997pneumonia} assumed that hospital-treated pneumonia patients with a very low probability of death would also have a very low probability of death if treated at home. \cite{caruana2015pneumonia} pointed 
out that this assumption may not hold, for example, in patients with a history of asthma. Due to the existing policy across hospitals to admit asthmatic pneumonia patients to the ICU, the aggressive treatment actually lowered their mortality risk from pneumonia compared to the general population.
While~\cite{caruana2015pneumonia} use this observation to argue for interpretable models,~\cite{schulam2017pneumonia} take it as motivation for causal models to ensure generalization.
% {\color{HighlightOrange} It is, however, unlikely that we would ever systematically infer the counterfactual, i.e., how asthma patients will fare without aggressive treatment in ICU, as it is unethical to withhold care deemed necessary by medical practitioners.
% Recent research on asthma and pneumonia even argues that the pneumonia etiology and outcomes are different for asthmatic patients than patients without this underlying illness~\citep{zaidi2019asthma}. 
% Note that this is the exact argument brought forward in the original study to exclude patients with a history of AIDS or a known positive HIV antibody titer~\citep{cooper1997pneumonia}.
% Hence, it even seems appropriate to also have excluded asthmatic patients from learning/application of any machine learning models in the first place.}

In another example, \cite{nestor2019records} trained predictive models on records from the MIMIC-III database between 2001 and 2002, and tested on data of subsequent years. When the underlying clinical information system changed in 2008, this caused fundamental changes in the recorded measurements and a significant drop in prediction quality of machine learning models trained on raw data. The predictive performance, however, remained surprisingly robust after aggregating the raw features into expert-defined clinical concepts.\footnote{Various measurements of the same biophysical quantity are grouped together.} If these clinical concepts reflect causal relationships, this example may  be viewed as empirical support for causal modeling.
% {\color{HighlightOrange} Moreover, the clinical aggregation also outperforms the raw feature representation in common MIMIC-III benchmark~\citep{johnson2016mimic}. Therefore, simply improving on said benchmark might even be the proper way to better approximate a robust (possibly causal) representation.}\\

In light of our results, it's worth finding theoretical explanations for why using all features, regardless of causality, has the best performance in typical tabular datasets. In this vein, \cite{rosenfeld2021online} 
point to settings where risk minimization is the right thing to do in theory. We seed the search for additional threotical explanations with a simple observation: If all domains are positive reweightings of one another, then the Bayes optimal predictor with respect to classification error in one domain is also Bayes optimal in any other domain. Standard models, such as gradient boosting or random forests, often achieve near optimal performance on tabular data with a relatively small number of features. In such cases, our simple observation applies and motivates a common sense heuristic: Do the best you can to approximate the optimal predictor on all available features.


